On Solving a Stochastic Shortest-Path Markov Decision Process as Probabilistic Inference

Previous work on planning as active inference addresses finite horizon problems and solutions valid for online planning. We propose solving the general Stochastic Shortest-Path Markov Decision Process (SSP MDP) as probabilistic inference. Furthermore, we discuss online and offline methods for planning under uncertainty. In an SSP MDP, the horizon is indefinite and unknown a priori. SSP MDPs generalize finite and infinite horizon MDPs and are widely used in the artificial intelligence community. Additionally, we highlight some of the differences between solving an MDP using dynamic programming approaches widely used in the artificial intelligence community and approaches used in the active inference community.

==> tex/00_abstract.tex <==


Previous work on planning as active inference addressed finite horizon problems. These solutions are useful for \textit{online} planning.  We address the general Stochastic Shortest-Path Markov Decision Process (SSP-MDP). In an SSP-MDP, the horizon is indefinite and unknown a priori. SSP-MDPs generalize finite and infinite horizon MDPs and are widely used in the artificial intelligence community. In this paper, we solve SSP-MDPs as probabilistic inference. We highlight the difference between online and offline MDP solvers. Furthermore, we discuss the difference between polices and (probabilistic) plans as well as states and temporal states. \textcolor{blue}{Finally, we provide guidelines on which methods would be most appropriate to use depending on the problems at hand. (IF THERE IS SPACE)}

% \thanks{asigijhgiygiuhiudf}

==> tex/01_intro.tex <==
\section{Introduction}

% Points I want to make:

% - Finite horizon problems vs indefinite
% - Probabilistic plan vs policy 
% - Online vs offline planning (most important for the 4 of us)
% - State vs temporal state 
% - Rewards vs max prob for reaching a state

% The core problem of this work is planning under uncertainty. The problem is typically modelled using a Markov decision process (MDP) (and rich models include with temporal logic specification \cite{plaku2012planning, lacerda2019probabilistic, hawes2017strands}). It is then solved using dynamic programming approaches. Such approaches assume discrete state-spaces, stationary problems and fully observable states \cite{kolobov2012planning}. We aim to translate the problem of planning with an MDP under a temporal logic specification to a problem of inference on a PGM. By modelling MDPs as PGMs, efficient approximate inference can be utilized. This is a principled way to find heuristic solvers. Additionally, the transition to more complex settings such as continuous and partially observable environments is straightforward from a PGM perspective \cite{toussaint2006probabilisticPOMDP, toussaint2006probabilistic}.



A core problem in the field of artificial intelligence (AI) is building agents capable of automated planning under uncertainty. Problems involving planning under uncertainty are typically formulated as an instance of a Markov Decision Process (MDP). At a high level, an MDP comprises 1) a set of world states, 2) a set of actions, 3) a transition model describing the probability of transitioning to a new state when taking an action in the current state, and 4) an objective function (e.g. maximizing the sum of rewards over a sequence of time steps). An MDP solution determines the agent’s actions at each decision point. An optimal MDP solution is one that optimizes the objective function. These are typically obtained using dynamic programming algorithms \cite{kolobov2012planning,sutton1998introduction}. 

Recent work based on the active inference framework \cite{friston2017active} poses the planning problem as a probabilistic inference problem. Several papers have been published showing connections between active inference and dynamic programming to solve an MDP \cite{kaplan2018planning_AIF,da2020relationship,da2020active}. However, the work in the two communities has a big gap. The problem being solved is not equivalent. In this paper, we highlight four key differences between solving an MDP using dynamic programming approaches and the work done in the active inference community. 


The first difference is regarding the idea of an \textit{indefinite horizon}. Consider an agent navigating a from a starting state to a goal state in a grid world where the outcome is uncertain (e.g. the 4x4 grid world in Figure \ref{fig:plan_vs_policy}). Before starting to act in the environment, there is no way for agent to know how many time steps it will take to reach the goal. In this problem, the horizon is finite but unknown a priori. This is referred to as an \textit{indefinite horizon}. Algorithms based on dynamic programming such as policy iteration, are valid for infinite, finite and indefinite horizons. However, work from active inference is only formulated for finite horizons. 

Dynamic programming approaches solve the so-called Stochastic Shortest-Path MDP which  assumes  an  indefinite  horizon. It can be shown than both finite and infinite MDPs are contained within Stochastic Shortest-Path MDPs \cite{kolobov2012planning}. Additionally, one can prove that an SSP MDP has an optimal deterministic solution. The definition and properties of an SSP MDP are disucced in Section \ref{sec:ssp_mdp}.

The second difference is the way the solution is formalized. In active inference, the solution to an MDP is computed as distribution over a sequence of actions and referred to as a policy \cite{catal2020learning,friston2017active,da2020active,da2020relationship}. To avoid confusion with the AI community, we refer to this as a \textit{probabilistic plan}. A classical plan is defined as sequence of actions in a deterministic model. A policy in the AI community refers to a mapping from states to actions. The difference between a policy, a plan and a probabilistic plan will be high-lighted further in Section \ref{subsec:plan_policy_prob_plan}. 


Since in active inference, a finite plan is computed, this makes it not suitable to solve an SSP MDP optimally. The horizon is unknown a priori and thus the optimal length of the plan can not specified. 

% Crucially, some work in the active inference community argues that is it more general since the consider stochastic policies. However, one can show that the optimal policy for an MDP is deterministic. 

The third difference is whether the solution is computed online or offline. An agent with an MDP can compute an optimal solution before executing actions in the  (offline planning), or while interacting with the environment (online planning). Planning as active inference can only be used for online planning since a plan is computed (a finite sequence of actions). The agent has to re-plan at every time-step depending on the outcome of the previous actions. However, dynamic programming approaches can be used for both online and offline planning. Since they compute a policy (a mapping from states to actions), it is sufficient to compute a policy offline and use it while interacting with the environment without any need to re-plan.


The fourth and final difference, is the how the state is defined. In dynamic programming, one reasons over the \textit{world states}. In the grid world example in Figure \ref{fig:plan_vs_policy}, this refers to a grid cell. This grid world has have 16 world states. In active inference, one reason about a\textit{ temporal state}. This is a random variable over all world states. The number of temporal states is dependant on how many timesteps the agents acts in the environment. The difference between world and temporal states is discussed in Section \ref{subsec:ssp_inference_definitions} and illustrated in Section \ref{subsec: temporal_vs_world_states}

% These two concepts can easily be mixed one when sampling based approaches are used such as in the reinforcement learning. This difference will be discussed in in section \ref{}. 


This paper has three contribution. First, we discuss an algorithm to solve a stochastic Shortest path Markov decision process using probabilistic inference. This is an MDP with an \textit{indefinite horizon}. Second, we highlight the gap between solving an MDP in the AI community and the active inference community as outlined by the four point in the introduction. Third, we provide guidelines on when to use different solution methods. For instance, when to compute policies (a mapping from states to actions) and when to compute probabilistic plans. 
\textcolor{blue}{There is no space really for last contribution so I can drop it. Or shorten something else and add this.}






==> tex/02_ssp_objective.tex <==
\section{SSP MDP}
\label{sec:ssp_mdp}

This section shortly discusses background information for planning under uncertainty. It discusses the Stochastic Shortest-Path Markov Decision Process (SSP-MDP). 

\subsection{Definition}
In this work we consider the the general Stochastic Shortest-Path MDP (SSP MDP). This model assumes an indefinite horizon, i.e. a horizon that is finite but unknown a priori. It can be shown than both finite and infinite MDPs are contained within Stochastic Shortest-Path MDPs \cite{kolobov2012planning}. The SSP MDP is defined as a tuple  $\langle\mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R}, \mathcal{G}\rangle$ where:
$\mathcal{S}$ is the finite set of all possible states of the system,
$\mathcal{A}$ is the finite set of all actions an agent can take,
$\mathcal{T}: \mathcal{S} \times \mathcal{A} \times \mathcal{S} \rightarrow[0,1]$ is a transition function specifying the probability $\mathcal{T}\left(s_{1}, a, s_{2}\right)$ of going to state $s_{2}$ whenever action $a$ is executed when the system is in state $s_{1}$, $\mathcal{R}: \mathcal{S} \times \mathcal{A} \times \mathcal{S} \rightarrow[0, \infty)$ is a reward function\footnote{The SSP MDP in \cite{kolobov2012planning} is defined in terms of cost functions. This means that our objective would be to maximize rewards rather the minimize costs} that gives a finite strictly positive reward $\mathcal{R}\left(s_{1}, a, s_{2}\right)>0$ incurred whenever the system goes from state $s_{1}$ to state $s_{2}$ as a result of executing action $a$, with the exception of transitions from a goal state, and
$ \mathcal{G} \subseteq \mathcal{S}$ is the set of all goal states s.t. for every $s_{g} \in \mathcal{G},$ for all $a \in \mathcal{A},$ and for all $s^{\prime} \notin \mathcal{G},$ the transition and reward functions obey $\mathcal{T}\left(s_{g}, a, s_{g}\right)=1, \mathcal{T}\left(s_{g}, a, s^{\prime}\right)=0,$ and $\mathcal{R}\left(s_{g}, a, s_{g}\right)=0$.


\textcolor{blue}{For Bruno: I stuck with a formulation based on rewards and added a footnote that Kolobov uses costs. }


\subsection{Computing an optimal policy}
The solution to an SSP MDP is referred to as a policy. It is a mapping from states to actions. From small problems this can be encoded as lookup table. For a stationary problem (one where the rewards and transition probabilities do not change over time), it is sufficient to compute the policy offline. This means that the agents computes the policy before acting in the environment, then uses the lookup table online (during execution time). 

The solution to an MDP is to find an optimal policy $\pi^*(s)$, that maximizes the expected reward $\mathbb{E}[\sum_{t=0}^{T} \gamma^T R_t]$, where $\gamma$ is discounting factor (an integer between 0 and 1). A discount factor of 1 is assumed for finite problems (such as our grid world). 

\textcolor{blue}{For Bruno: You wrote ``for an SSP you need to minimise. all of this is a bit on the imprecise side, please spend some time making it neater". I am assuming it that remains a max since I am working with rewards, right?}

\subsection{Properties of the optimal policy}
A proper policy is a policy that is guaranteed to bring the agent to a goal state from any other state. For a SSP MDP there exists at least one proper deterministic policy according to the assumptions followed in \cite{kolobov2012planning}.
Additionally, it can be proven that each SSP MDP has an optimal deterministic policy independent of time. Thus the claims made in \cite{da2020relationship} about active inference being more general since it computes stochastic policies are unjustified when solving an MDP. However, these results do not hold in partially observable cases or in the presence of uncertain models. But in the SSP MDP defined above (which is vastly used in the AI community), there always exists a deterministic optimal policy. 


\subsection{Policies, plans and probabilistic plans}
\label{subsec:plan_policy_prob_plan}

Classical planning algorithms computes plans: a sequence of actions. An algorithm like A* or Dijkstra's algorithm \cite{cormen2009introduction} can be used to find the optimal path from a stating state to a goal state given a deterministic world. Crucially, this solution can be computed offline (without interactions with the environment). In a stochastic world, this does not work since the agent can not predict in which states it will end up. However, one can use deterministic planning algorithms for stochastic environments if you plan and re-plan online. This means, the agent uses the world and plans a sequence of actions online (while interacting with the environment). Determinization-based methods  have found some success in the past including FF-replan \cite{yoon2007ff-replan}

Active inference approaches computes a \textit{probabilistic plan}. The active inference literature calls this as a policy; however, we refer use a different term to avoid confusion with the AI literature.\footnote{The distinction between a plan and a policy when using active inference has been briefly discussed in \cite{millidge2020relationship}. Additionally, others methods computing plans as probabilistic inference have been proposed before active inference in \cite{attias2003planning,verma2006goal}} In active inference, the agents computes a finite plan while interacting with the environment. However, rather than assuming a deterministic world (like FF-replan \cite{yoon2007ff-replan}), the probabilities are taken into account. The agent computes a distribution over plan. This can be shown to compute the optimal solution to an MDP (when planning online). 

Finally, a policy is a mapping from states to actions. I.e. for every state, the agents has a preferred actions to take. Policies can be stochastic or time-dependent; however, for an SSP MDP the optimal policy if deterministic and independed of time. An agent can compute a policy offline and simply use it online without needing any additional computation while interacting with the environment. The difference between a plan and policy is illustrated in Figure \ref{fig:plan_vs_policy}. 

To conclude, a plan or a probabilistic plans can only be used for online planning. Probabilistic plans (as used in active inference) find an optimal solution when used to plan online. A policy also provides an optimal solution and can be computed offline or online. 

% A discussion on when to use policies and plans is presented in ***. 











==> tex/03_policy_iteration.tex <==
\section{Solving an SSP MDP using Policy iteration}

Finding the optimal policy can achieved using a \textit{policy iteration} algorithm. Policy iteration consists of two steps. The first step is policy evaluation, which computes a value function $v_{\pi}(s)$ given a policy $\pi$ for every world state $s$. The value of a state $s$ under policy $\pi$ is the total expected reward that an agent, starting out in $s$, accumulated before it reaches a goal state $g$. Psuedo code for policy iteration is given in Algorithm \ref{algo: Standard policy evaluation} in the appendix. The second step is policy improvement. In this step the state-action value function $Q(s,a)$ is computed. Afterwards, a greedy update is performed for the actions the maximizes $Q(s,a)$. Policy improvement is given in algorithm \ref{algo:policy_improvement} in the appendix. Iterating between policy evaluation and policy improvement until convergence results in the policy iteration algorithm. 


\subsection{Termination criterion}

In the policy evaluation step, one iterates through the states to update the value $v_{\pi}(s)$ for every policy until a termination criterion is met. Most commonly, an $\epsilon$-greedy criterion is used. This means that we stop iterating though the state space once the maximum difference in $v_{\pi}(s)$ for any $s$ is smaller than a number $\epsilon$ (as given in algorithm \ref{algo: Standard policy evaluation}). An alternative is \textit{truncated policy iteration}. Here we iterate through the state space $T_{max}$ times (as given in algorithm \ref{algo:truncated_policy_evaluaiton}) then perform policy improvement. The probabilistic inference algorithm presented in this paper will be equivalent to truncated policy iteration. 
% However, one can easily design a version equivalent to $\epsilon$-greedy policy iteration. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







% $$
% \begin{array}{l}
% \hline \text { Algorithm 3: Policy Improvement } \\
% \hline \text { Input: MDP, value function } V \\
% \text { Output: policy } \pi^{\prime} \\
% \text { for } s \in \mathcal{S} \text { do } \\
% \mid \begin{array}{l}
% \text { for } a \in \mathcal{A}(s) \text { do } \\
% \mid \quad Q(s, a) \leftarrow \sum_{s^{\prime} \in \mathcal{S}, r \in \mathcal{R}} p\left(s^{\prime}, r \mid s, a\right)\left(r+\gamma V\left(s^{\prime}\right)\right) \\
% \text { end } \\
% \qquad \pi^{\prime}(s) \leftarrow \arg \max _{a \in \mathcal{A}(s)} Q(s, a) \\
% \text { end } \\
% \text { return } \pi^{\prime}
% \end{array}
% \end{array}
% $$



% Finite-horizon and infinite-horizon discounted MDPs are located at the opposite ends of a spectrum — the former assume the number of time steps to be limited and known; the latter assume it to be infinite. This suggests a natural third possibility, problems with finite but unknown horizon. Imagine, for instance, a space shuttle trying to enter Earth’s atmosphere and land after a
% mission. During every revolution around Earth, the shuttle can either choose to land or continue on to the next revolution, e.g., due to bad weather. In theory, the shuttle can orbit in space forever. However, poor weather conditions cannot persist for too long, so with overwhelming probability the shuttle will land after some finite but a priori unknown number of attempts, if controlled optimally. More formally, we can think of indefinite-horizon problems as processes that, under every optimal policy, inevitably reach some terminal state. As long as the process has not reached a terminal state, it incurs negative reward, i.e., cost (in the shuttle example, the cost can be crew fatigue). Once the target state is reached, no more cost is incurred. Thus, the total expected cost of any optimal policy in such an MDP should be finite even without a discount factor. In spite of this fairly straightforward logic, precisely stating a set of conditions under which
% an optimal policy exists in the presence of an indefinite horizon is tricky, and we devote the entire next section to its derivation.

==> tex/04.1_dynamic_programming_or_inference.tex <==
\section{Connections between the two views}

\subsection{Exact relationship between policy iteration and planning as probabilistic inference}
The $\beta$ messages computed during backward propagation are the value functions for a single MDP of finite time. The full value function is the mixture of the $\beta$s,
$V_{\pi}(i) = 1/(1 - \gamma) \sum_T P(T) \beta_T(i)$, when a discount time prior is chosen. The same applies to the relationship between the Q-value function. Hence, the E-step essentially performs a policy evaluation which yields the classical value function. Given this relation to policy evaluation, the M-step performs a policy update which (for the greedy M-step) is the standard policy improvement in Policy Iteration. Thus, the EM-algorithm using exact inference is effectively equivalent to Policy Iteration (also w.r.t. convergence) but computes the necessary quantities in a different way.


One unanswered question is when we stop computing the backward messages $\beta$. Previous work has usually set a maximum horizon and computed messages up to that point. From this perspective, the planning as inference algorithm presented here is exactly equivalent to a \textit{truncated policy iteration} algorithm (which is discussed in the previous section). Modifications can be made for an algorithms equivalent to $\epsilon$-greedy policy iteration. 




\subsection{World states vs temporal states}
\label{subsec: temporal_vs_world_states}
In dynamic programming, one reasons over the world states (e.g. a grid cell in a grid world). In probabilistic inference, one reasons about a\textit{ temporal state}. This is a random variable over all world states. A posterior of the temporal state is a distribution over all world state and provides information about where the agent is likely to be at time-step $t$. An illustration of the difference is given in Figure \ref{fig:tempral_and_world_state}. 






% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=\textwidth]{world.JPG}
%     \caption{Temporal state vs world state}
%     \label{fig:tempral_and_world_state}
% \end{figure}



% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=\textwidth]{optimal_v.JPG}
%     \caption{Optimal value function}
%     \label{fig:optimal_v}
% \end{figure}


==> tex/04_planning_as_inference.tex <==
\section{Solving a SSP MDP as probabilistic inference}
\label{sec:solving_ssp_as_inference}

In this section we discuss an approach for solving an SSP MDP as probabilistic inference. Modifications of this approach have been presented in \cite{toussaint2006probabilistic,toussaint2006probabilisticPOMDP} and successfully applied to solve problems of planning under uncertainty, e.g. \cite{kumar2015probabilistic,toussaint2008hierarchical}. 


\subsection{Definitions}
\label{subsec:ssp_inference_definitions}
The definition of an SSP MDP includes a set of world states $\mathcal{S}$ and actions $\mathcal{A}$. In probabilistic inference we instead reason about \textit{temporal} states and actions. A temporal state $s_t$ is a random variable defined over all world states. It conceptually is the state the agent will visit at the time-step $t$. For the grid world in Figure \ref{fig:plan_vs_policy}, there are 16 world states but the number of temporal states is unknown a priori since the horizon is unknown. 


The transition probability is defined as a probability distribution over temporal states and actions as $P(s_{t+1}|a_t, s_t)$. If the random variables are fixed to specific world states $i$ and $j$ and an action $a$, the transition probability $P(s_{t+1}=j|a_t=a, s_t=i)$ would be equivalent to the transition function $\mathcal{T}$ defined for an SSP MDP. The probability of taking a certain action is a an state is parameterized by a policy $\pi$ as $P(a_t=a|s_t=i;\pi) = \pi_{ai}$. This policy is defined exactly the same as in the case of an SSP MDP.

The reward function $P(r_t|s_t, a_t)$ is defined differently. The temporal reward variables $r_t$ are defined as binary random variables $r_t \in \{0, 1\}$. Translating an arbitrary reward function to temporal rewards can be done by scaling reward function $\mathcal{R}$ between the minimum reward (min($\mathcal{R}$)) and maximum reward (max($\mathcal{R}$)) as: 

$$
P(r_t \mid a_t, s_t)=\frac{\mathcal{R}(a, s)-\min (\mathcal{R})}{\max (\mathcal{R})-\min (\mathcal{R})}.$$

Now we can reason about the maximum reward as one where $P(r_t = 1, s_t, a_t) = 1$ and the minimum reward as $P(r_t = 1) = 0$. Any other reward will have a probability in-between according to its magnitude. 


Finally, we model the horizon. We temporal states and actions are considered up to the end of the horizon $T$. However, the horizon is generally unknown. We thus model $T$ itself as a random variable. combining all this information we can define the SSP MDP using a probabilistic model.


% States and actions are random variables. 
% We have transition probability 
% We have a policy 
% The rewards needs to be modelled as a random variable. We do it binary. Explain how that happens. 
% We need to stop at some T, but we don't know it. So we model it as a random variable. This one of the main differences with AIF work. 






\subsection{Mixture of finite MDPs}
In this section we define the SSP MDP in terms of a mixture of finite MDPs with only a final reward variable. Given every horizon (for instance $T = 1$) the finite MDP can be given as $P\left(r, s_{0: T}, a_{0: T} \mid T ; \boldsymbol{\pi}\right)$. Note that we dropped the time-index for $r_t$ since there is only one reward variable now.  This model can be factorized as

$$
\begin{array}{r}
P\left(r, s_{0: T}, a_{0: T} \mid T ; \boldsymbol{\pi}\right)= P\left(r \mid a_{T}, s_{T}\right) P\left(a_{0} \mid s_{0} ; \boldsymbol{\pi}\right) \\ P\left(s_{0}\right) 
\cdot \prod_{t=1}^{T} P\left(a_{t} \mid s_{t} ; \boldsymbol{\pi}\right) P\left(s_{t} \mid a_{t-1}, s_{t-1}\right)
\end{array}
$$




To reason about the full MDP, we consider the mixture model of the joint given by the joint probability distribution
$$
P\left(r, s_{0: T}, a_{0: T}, T ; \boldsymbol{\pi}\right)=P\left(r, s_{0: T}, a_{0: T} \mid T ; \boldsymbol{\pi}\right) P(T)
$$
where $P(T)$ is a prior over the total time, which we choose proportional to the discounting factor $\gamma$, $P(T)=$ $\gamma^{T}(1-\gamma).$ If $\gamma$ is set to 1, we consider a flat prior. An graphical representation of the whole MDP (full mixture model) and the finite MDPs is given in Figure \ref{fig:mixture_model}.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=\textwidth]{images/mixture_model.JPG}
%     \caption{An illustration of a mixture of finite MDPs with a terminal reward and the full MDP.}
%     \label{fig:mixture_model}
% \end{figure}



% Now we can consider the reward variable $r$ as observations, condition on the start state, and define the likelihood for a single finite-time MDP,
% $$
% L_{T}^{\pi}(i)=P\left(r=1 \mid s_{0}=i, T ; \boldsymbol{\pi}\right)=\mathrm{E}\left\{r \mid s_{0}=i, T ; \boldsymbol{\pi}\right\}
% $$
% and for the full misture of MDPs,
% $$
% \begin{aligned}
% L^{\pi}(i) &=P\left(r=1 \mid s_{0}=i ; \boldsymbol{\pi}\right) \\
% &=\sum_{T} P(T) \mathrm{E}\left\{r \mid s_{0}=i, T ; \boldsymbol{\pi}\right\}
% \end{aligned}
% $$
% This likelihood is, for the discounted time prior $P(T)=\gamma^{T}(1-\gamma),$ proportional to the espected future return, $^{2}$
% $$
% L^{\pi}(i)=(1-\gamma) V^{\pi}(i)
% $$



\subsection{A complete optimal policy}
Our objective is now to solve for the the policy that maximizes the expected reward ($P(r=1)$). Like policy iteration, We do not assume any knowledge about the initial state. Expectation-Maximization\footnote{An expectation-maximization algorithm can be viewed as algorithm performing free-energy minimization \cite{murphey_book,koller_book}. In the E-step, the free-energy is computed and the M-step updates the parameters to minimize the free-energy.} can be used to find the optimal parameters of our model. These parameters are the the policy $\pi$. All action and state variables are hidden variables. The E-step will, for a given $\pi$, compute posteriors over state-action sequences. The M-step then adapts the model parameters $\pi$ to optimize the expected likelihood w.r.t. the quantities calculated in the E-step.

\textbf{E-step: a backwards pass in all finite MDPs.}

We use the simpler notation $p(j \mid a, i)=P\left(s_{t+1}=j \mid a_{t}=a, s_{t}=i\right)$ and
$p(j \mid i ; \boldsymbol{\pi})=P\left(s_{t+1}=j \mid s_{t}=i ; \boldsymbol{\pi}\right)=\sum_{a} p(j \mid a, i) \pi_{a i} .$
Further, as a ``seed" for backward propagation, we define
$$
\begin{aligned}
{\beta}_0(i) &=P\left(r=1 \mid x_{T}=i ; \boldsymbol{\pi}\right) =\sum_a P\left(r=1 \mid a_{T}=a, x_{T}=i\right) \pi_{a i}.
\end{aligned}
$$

This essentially is the immediate reward when following a policy $\pi$. It is the expected reward if there is only one time-step remaining. From here on, we can recursively compute all the other backward messages. We use the index $\tau$ to indicate a backwards counter. This means that $\tau + t = T$, where $T$ is total unknown horizon.


% \begin{equation}
% \begin{aligned}
$$
\beta_{\tau}(i) =P\left(r=1 \mid x_{T-\tau}=i ; \boldsymbol{\pi}\right) =\sum_{j} p(j \mid i ; \boldsymbol{\pi}) \beta_{\tau-1}(j).
$$
% \end{aligned}
% \end{equation}

Intuitively, the backward messages indicate the expected reward, if one receives only a reward at the last time step. So $\beta_2$, is the expected reward if the agent follows the policy $\pi$ for two time-steps and only receives a reward after that. Using these messages, we can compute a value function dependant on time, actions and states gives as: 

$$
\begin{aligned}
&q_{t \tau}(a, i)=P\left(r=1 \mid a_{t}=a, s_{t}=i, T=t+\tau ; \boldsymbol{\pi}\right) \\
&=\left\{\begin{array}{ll}
\sum_{j} p(j \mid i, a) \beta_{\tau-1}(j) & \tau>1 \\
P\left(r=1 \mid a_{T}=a, s_{T}=i\right) & \tau=0
\end{array}\right.
\end{aligned}
$$

Multiplying with the time prior and eliminating the total time we get the state-action value-function 
$$
\begin{aligned}
&P\left(r=1 \mid a_{t}=a, s_{t}=i ; \boldsymbol{\pi}\right) =\frac{1}{C} \sum_{\tau} P(T=t+\tau) q_{\tau}(a, i)
\end{aligned}
$$
where $C$ is a normalization constant. This quantity is the probability of getting a maximum reward given a state and action. It is similar to the $Q(s, a)$ function computed in policy iteration (algorithm \ref{algo:policy_improvement}).


\textbf{M-step: the policy improvement step}


The standard M-step in an EM-algorithm maximizes the expected complete log-likelihood with respect to the new parameters $\pi^*$. Given the knowledge that the optimal policy for an MDP is deterministic, a greedy M-step can be used. 

\begin{equation}
\begin{aligned}
&\pi^{*} =\underset{a}{\operatorname{argmax}} P\left(r=1 \mid a_{t}=a, s_{t}=i ; \boldsymbol{\pi}\right)
\end{aligned}
\end{equation}

This update converges much faster than a standard M-step update. Work in \cite{da2020relationship} argues that active inference is more general since it considers stochastic policies. Here an M-step can be used to to obtain a stochastic policy as well. However, the is unnecessary since the optimal policy is deterministic. In conclusion, a greedy M-step is faster to converge but still guarantees an optimal policy. 



==> tex/05_resutls.tex <==
\section{Results}

\textcolor{blue}{For Bruno: I have some results for max-prob and other things here but I didn't have space to discuss them. Should I just leave this empty or maybe add some results showing that Planning as inference and policy iteration do pretty much the same thing. Just say hey here are a couple of grid worlds and they converge both in this many time step ...etc}

==> tex/06_dicussion_conclusion.tex <==
% \section{Discussion and conclusion}

